Improving text classification with vectors of reduced precision

This paper presents the analysis of the impact of a floating-point number precision reduction on the quality of text classification. The precision reduction of the vectors representing the data (e.g. TF-IDF representation in our case) allows for a decrease of computing time and memory footprint on dedicated hardware platforms. The impact of precision reduction on the classification quality was performed on 5 corpora, using 4 different classifiers. Also, dimensionality reduction was taken into account. Results indicate that the precision reduction improves classification accuracy for most cases (up to 25% of error reduction). In general, the reduction from 64 to 4 bits gives the best scores and ensures that the results will not be worse than with the full floating-point representation.

==> acronyms.tex <==
% CERN
\newacronym{LHC}{LHC}{Large Hadron Collider}
\newacronym{CERN}{CERN}{the European Organization for Nuclear Research}
\newacronym{PM}{PM}{Post Mortem}
\newacronym{PMS}{PM System}{\glsentrylong{PM} System}
\newacronym{PMF}{PM Framework}{\glsentrylong{PM} Framework}
\newacronym{LEP}{LEP}{Large Electron-Positron Collider}
\newacronym{PS}{PS}{Proton Synchrotron}
\newacronym{SPS}{SPS}{Super Proton Synchrotron}
\newacronym{ATLAS}{ATLAS}{A Toroidal LHC ApparatuS}
\newacronym{CMS}{CMS}{Compact Muon Solenoid}
\newacronym{ALICE}{ALICE}{A Large Ion Collider Experiment} \newacronym{LHCb}{LHCb}{Large Hadron Collider beauty experiment}
\newacronym{SUSY}{SUSY}{SUperSYmmetry}
\newacronym{SSB}{SSB}{Spontaneous Symmetry Breaking}
\newacronym{QPS}{QPS}{Quench Protection System}
\newacronym{SDDS}{SDDS}{Self-Describing Data Set}
\newacronym{MTF}{MTF}{Magnet Test Folder}
\newacronym{ELQA}{ELQA}{ELectrical Quality Assurance}

\newacronym{TE-MPE-EE}{TE-MPE-EE}{Technology Department --Machine Protection and Electrical Integrity group -- Electrical Engineering group}

% Deep Learning
\newacronym{DL}{DL}{Deep Learning}
\newacronym{LSTM}{LSTM}{Long Short-Term Memory}
\newacronym{GRU}{GRU}{Gated Recurrent Unit}
\newacronym{RMSE}{RMSE}{Root-Mean-Square Error}
\newacronym{RNN}{RNN}{Recurrent Neural Network}
\newacronym{ASIC}{ASIC}{Application-Specific Integrated Circuit}
\newacronym{FPGA}{FPGA}{Field-Programmable Gate Array}
\newacronym{FNN}{FNN}{Feed-forward Neural Network}
\newacronym{CNN}{CNN}{Convolutional Neural Network}

==> contents-10-system-description.tex <==
\section{System description}
\label{section:system_description}

As described in \cite{wielgosz2016opencl}.
